Large Scale Holistic Video Understanding

Video recognition has been advanced in recent years by benchmarks with rich annotations. However, research is still mainly limited to human action or sports recognition - focusing on a highly specific video understanding task and thus leaving a significant gap towards describing the overall content of a video. We fill this gap by presenting a large-scale "Holistic Video Understanding Dataset"~(HVU). HVU is organized hierarchically in a semantic taxonomy that focuses on multi-label and multi-task video understanding as a comprehensive problem that encompasses the recognition of multiple semantic aspects in the dynamic scene. HVU contains approx.~572k videos in total with 9 million annotations for training, validation, and test set spanning over 3142 labels. HVU encompasses semantic aspects defined on categories of scenes, objects, actions, events, attributes, and concepts which naturally captures the real-world scenarios. We demonstrate the generalization capability of HVU on three challenging tasks: 1.) Video classification, 2.) Video captioning and 3.) Video clustering tasks. In particular for video classification, we introduce a new spatio-temporal deep neural network architecture called "Holistic Appearance and Temporal Network"~(HATNet) that builds on fusing 2D and 3D architectures into one by combining intermediate representations of appearance and temporal cues. HATNet focuses on the multi-label and multi-task learning problem and is trained in an end-to-end manner. Via our experiments, we validate the idea that holistic representation learning is complementary, and can play a key role in enabling many real-world applications.

==> intro_rel_BACKUP.tex <==
\section{Abstract Old}

There are lots of works in video recognition field
focusing on specific video understanding tasks, such as, action recognition, scene understanding, etc. There have been great achievements in such tasks, however, there has not been enough attention toward the holistic video understanding task as a problem to be tackled. Current systems are expert in some specific fields of the general video understanding problem. However, for real world applications, such as, analyzing multiple concepts of a video for video search engines and media monitoring systems or providing an appropriate definition of the surrounding environment of an humanoid robot, a combination of current
state-of-the-art methods should be used.

In this work, we introduce the holistic video understanding
as a new challenge for the video understanding efforts. This challenge
focuses on the recognition of scenes, objects, actions, attributes, and events in the real world user generated videos. To be able to address such tasks, we also introduce our new dataset named Holistic Video Understanding (HVU) dataset that is organized hierarchically in a semantic taxonomy of holistic video understanding. Almost all of real-wold conditioned video datasets are targeting human action or sport recognition. 

We also propose our new video recognition deep neural network called HATnet which is an efficient pipeline to understand different concept categories in videos in multi-task and multi-label recognition fashion. HATnet also achieved outstanding performance on existing video datasets like Kinetics and UCF101.




%%%%%%%%% BODY TEXT
\section{Introduction}

A video is much more than the depiction of a human action. It often portrays a scene or an environment (an office, a basketball court, a beach), and includes background objects (a picture, a door, a bus) as well as objects manipulated or utilized by a person (e.g., lipstick, a tennis racquet, a wrench). An action label provides a human-centric description of the video but ignores this relevant contextual information. Yet, today most existing video classification datasets contain only human action tags. While a few object-centric video datasets have been proposed [28, 14], there is no established video benchmark integrating joint recognition of scenes, objects and actions. To the best of our knowledge the only exceptions are perhaps YouTube-8M [1] and Charades [31], where some of the classes are pure actions (e.g., wrestling), some represent objects (e.g., bicycle), and some denote “objects in action” (e.g., drinking from a cup). Unlike in these prior datasets, where contextual information (scenes and objects) is coupled with action categorization in the form of flat classification, we propose a dataset that integrates scene, object, and action categorization in the form of multi- task classification, where labels are available for each of these three aspects in a video. This makes it possible to quantitatively assess synergy among the three tasks and leverage it during modeling.

Furthermore, this multi-task formulation recasts video understanding as a comprehensive problem that encompasses the recognition of multiple semantic aspects in the dynamic scene.

\textbf{$-$ Single label vs Multi label.}

Finally, we argue that a single class label per task is often not sufficient to describe the content of a video. Even a single frame may contain multiple prominent objects; the addition of a temporal dimension makes multi-label even more important for video than for images.... as they mostly contain prototypical examples for which a single-label assumption is reasonable.






\textbf{$-$ Better generalization just like ImageNet dataset based trained model.}

\textbf{$-$ The use of large-scale datasets is extremely important when using deep convolutional neural networks (CNNs), which have massive parameter numbers, and the use of CNNs in the field of computer vision has expanded signifi- cantly in recent years. ImageNet [4], which includes more than a million images, has contributed substantially to the creation of successful vision-based algorithms. In addition to such large-scale datasets, a large number of algorithms, such as residual learning [10], have been used to improve image classification performance by adding increased depth to CNNs, and the use of very deep CNNs trained on Im- ageNet have facilitated the acquisition of generic feature representation. Using such feature representation, in turn, has significantly improved the performance of several other tasks including object detection, semantic segmentation, and image captioning.}

\textbf{$-$ One of the unexpected benefits of the ImageNet challenge has been the discovery that deep architectures trained on the 1000 images of 1000 categories, can be used for other tasks and in other domains. One of the early examples of this was using the fc7 features from a network trained on ImageNet for the PASCAL VOC classification and detection challenge [10]. Furthermore, improvements in the deep architecture, changing from AlexNet to VGG-16, immediately fed through to commensurate improvements in the PASCAL VOC performance [23]. Since then, there have been numerous examples of ImageNet trained architectures warm starting or sufficing entirely for other tasks, e.g. segmentation, depth prediction, pose estimation, action classification.}

\textbf{$-$ However, despite the explosion of video data, the ability to automatically recognize and under- stand human activities is still rather limited. This is primarily due to impeding challenges inherent to the task, namely the large variability in execution styles, complexity of the visual stimuli in terms of camera motion, background clut- ter and viewpoint changes, as well as, the level of detail and number of activities that can be recognized. An im- portant limitation that hinders the performance of current techniques is the state of existing video datasets and bench- marks available to action/activity recognition researchers.}

It is useful to fairly represent in the dataset the distri- bution of videos on the Internet. By doing so, models trained on the dataset can be directly applied to understand and recognize popular concepts in everyday Internet videos.





\textbf{$-$ In the video domain, it is an open question whether training an action classification network on a sufficiently large dataset, will give a similar boost in performance when applied to a different temporal task or dataset. The challenges of building video datasets has meant that most popular benchmarks for action recognition are small, having on the order of 10k videos.}

\textbf{$-$ In spite of this fact, most computer vision algorithms for human activity understand- ing are benchmarked on datasets that cover a limited num- ber of activity types. In fact, existing databases tend to be specific and focus on certain types of activities i.e. sports, cooking or simple actions. Typically, these datasets have a small number of categories (around 100), a small number of samples (short clips) per category (around 100), and limited category diversity.}

\textbf{$-$ To date, the video datasets available for action recognition have been relatively small when compared with image recog- nition datasets. Representative video datasets, such as UCF- 101 [21] and HMDB-51 [17], can be used to provide realistic videos with sizes around 10 K, but even though they are still used as standard benchmarks, such datasets are obviously too small to be used for optimizing CNN representations from scratch. In the last couple of years, ActivityNet [5], which is a somewhat larger video dataset, has become available, and its use has make it possible to accomplish additional tasks such as untrimmed action classification and detection, but the number of action instances it contains is still limited. More than 300 K videos have been collected for the Kinetics dataset, which means that the scale of video datasets has begun to approach that of image datasets.}




\textbf{$-$ HUV has two orders of magnitude more data, with 400 human action classes and over 400 clips per class, and is collected from realistic, challenging YouTube videos.}

\textbf{$-$ We provide an analysis on how current architectures fare on the task of action classification on this dataset and how much performance improves on the smaller benchmark datasets after pre-training on HUV.}

\textbf{$-$ We introduce a new spatio-temporal architecture making it possible to learn seamless spatio-temporal feature extractors from video while leveraging successful ImageNet architecture designs and even their parameters.}




In this work we introduce a new video dataset aimed at advancing research on video understanding. We name the dataset Scenes-Objects-Actions (SOA), as each video is annotated with respect to three different aspects: scenes, objects, and actions. Our objective is to introduce a benchmark that will spur research in video understanding as a comprehensive, multi-faceted problem.

\textbf{$-$ In this paper we aim to provide an answer to this question using the new Kinetics Human Action Video Dataset [16], which is two orders of magnitude larger than previous datasets, HMDB-51 [18] and UCF-101 [27]. Kinetics has 400 human action classes with more than 400 examples for each class, each from a unique YouTube video.}

\textbf{$-$ One of the most important aspects of ActivityNet is that it is structured around a semantic ontology which organizes activities ac- cording to social interactions and where they usually take place. It provides a rich activity hierarchy with at least four levels of depth. To the best of our knowledge, ActivityNet is the first database for human activity recognition organized under a rich semantic taxonomy.}

\textbf{$-$ Our experimental strategy is to analyze their transfer behavior by first pre- training the models on HUV datasset  and then fine-tuning each on HMDB-51 and UCF-101, in comparison to models trained on Kinetics. The results suggest that there is always a boost in performance by pre-training on multi-task learning via HUV dataset. }


The final dataset includes 562K videos with 3.64M annotations spanning 49 categories for scenes, 356 for objects, 148 for actions, and naturally captures the long tail distribution of visual concepts in the real world.

We compare SOA with existing datasets and discuss various factors that impact the performance of transfer learning. A key- feature of SOA is that it enables the empirical study of correlation among scene, object and action recognition in video.

We present results of this study and further analyze the potential of using the information learned from joint task to improve and learn better features towards challenging holistic video analysis for a a more comprehensive understanding in comparison to single-label classification of video data.







\textbf{$-$ Based on these findings, we introduce a new model that has the capacity to take advantage of pre-training on Kinetics, and can achieves a high performance. The model is termed as ``HAV Network" which fuses 2D and 3D architectures into one by combining intermediate representations from temporal and visual cues, leading to a robust spatio-temporal representation.}

More specifically, can the use of 3D CNNs trained on Kinetics produces significant progress in action recognition and other various tasks?  To achieve such progress, we consider that Kinetics for 3D CNNs should be as large-scale as ImageNet for 2D CNNs, though no previous work has examined enough about the scale of Kinetics. 

To our best knowledge, this is the first work to focus on the training of very deep 3D CNNs from scratch for video understanding and beating dataset trained on Kinetics, thus clearly showing the impact of HVU achieved better performance.

\textbf{$-$ Our HUVnet obtains performance far exceeding the state-of-the-art, after pre-training on HUV dataset.}

\textbf{$-$ Our experimental strategy requires no ImageNet pre-trained image classification architecture as back bone.}





\section{Related Works}

\noindent
\textbf{Action Recognition with ConvNets:} %/without
%Over the last two decades, multitude of action recognition techniques in videos have been proposed by the vision community. Among the hand-engineered ones with that could model effectively the  appearance and motion representations across frames in videos are HOG3D~\cite{hog3d}, SIFT3D~\cite{sift3d}, HOF~\cite{hof}, ESURF~\cite{esurf} and MBH~\cite{mbh}, iDTs~\cite{idt} and more. Despite their good performance, they have several shortcomings, they are computationally expensive and lack scalability to capture semantic concepts for large scale dataset.  To overcome such issues, several other techniques were proposed to model the temporal structure in an efficient way, such as the actom sequence model~\cite{actoms}; temporal action decomposition~\cite{temporalactiondecomposition}; dynamic poselets~\cite{dynamicposelets}; ranking machines~\cite{basura}.
With Convolutional Neural Networks (ConvNets) the vision community has successfully made huge leaps forward in several sub-fields of vision and has outperformed hand-engineered representations by a significant margin particularly for action recognition. End-to-end ConvNets have been introduced in~\cite{pooling,karpathy,twostream,c3d,tsn}  to exploit the appearance and the temporal information. These methods operate of 2D (individual image-level) or 3D (video-clips or snippets of $K$ frames).  In the 2D setting, spatial and/or temporal information are modeled via LSTMs/RNNs to capture long-term motion cues~\cite{lstm1,n3d}, or via feature pooling and encoding methods  using Bilinear models~\cite{tle}, Vector of Locally Aggregated Descriptors~(VLAD)~\cite{actionvlad}, and Fisher vector encoding~(FVs)~\cite{fishernet}. While, in the 3D settings, the input to the network consists of either RGB video clips or stacked optical-flow frames to capture the long-term temporal information. The filters and pooling kernels for these architectures are 3D (x, y, time) i.e. 3D convolutions~($s \times s\times d$)~\cite{n3d} where $d$ is the kernel temporal depth and $s$ is the kernel spatial size. Simonyan et al.~\cite{twostream}  use two-stream 2D ConvNets cohorts of RGB images and a stack of 10 optical-flow frames as input. Tran et al.~\cite{c3d} on the other side explored 3D ConvNets with fixed kernel size of  $3\times 3 \times 3$, where spatio-temporal feature learning for clips of 16 RGB frames was performed. In this way, they avoid to calculate the optical flow explicitly and still achieve good performance. Further, in~\cite{res3d,r2plus1} Tran et al. extended the ResNet architecture with 3D convolutions. In~\cite{pooling} Feichtenhofer et al. propose 3D pooling.  Sun et al.~\cite{sun3d} decomposed the 3D convolutions into 2D spatial and 1D temporal convolutions. Wang et al.~\cite{tsn} propose to use sparsely sampled non-overlapping frames from the whole clip as input for both spatial and temporal streams and then combine their scores in a late fusion approach.  Carreira et al.~\cite{i3d} propose converting a pre-trained 2D ConvNet~\cite{googlenet} to 3D ConvNet by inflating the filters and pooling kernels with an additional temporal dimension $d$. All these architectures have fixed temporal 3D convolution kernel depths throughout the whole architecture. In T3D~\cite{t3d}, Diba et al. propose temporal transition layer that models variable temporal convolution kernel depths over shorter and longer temporal ranges. Further in~\cite{stcnn}, Diba et al. propose spatio-temporal channel correlation that models correlations between channels of a 3D ConvNets wrt. both spatial and temporal dimensions. In contrast to these prior works, our work differs substantially in scope and technical approach. We propose an architecture to learn dynamic motion filters for modeling an effective internal motion representation in order to adaptively extract informative motion features conditioned on a video-specific basis to improve action recognition.

%Finally, it is worth noting the self-supervised learning works on ``harvesting" training data from unlabeled sources for action recognition.  Fernando~\etal~\cite{Odd-one} and Mishra~\etal~\cite{Shuffle} shuffle the video frames and treat them as positive/negative training data for reordering video frames; Wei et al.~\cite{wei} divides a single clip into non-overlapping 10-frame chunks, and then predict the ordering task; Ng et al.~\cite{actionflow} estimates optical flow while recognizing actions. We compare all these methods against our unsupervised future frame prediction based ConvNet training. 


One of the popular approaches to CNN-based action recognition is the use of two-stream CNNs with 2D con- volutional kernels. In their study, Simonyan et al. proposed a method that uses RGB and stacked optical flow frames as appearance and motion information, respectively [20], and showed that combining the two-streams has the abil- ity to improve action recognition accuracy. Since that study, numerous methods based on the two-stream CNNs have been proposed to improve action recognition perfor- mance [6, 7, 8, 27, 28, 29].

Unlike the abovementioned approaches, we focused on CNNs with 3D convolutional kernels, which have recently begun to outperform 2D CNNs through the use of large-scale video datasets. These 3D CNNs are intuitively effective because such 3D convolution can be used to directly extract spatio-temporal features from raw videos. For example, 

Meanwhile, Kay et al. showed that the results of 3D CNNs trained from scratch on their Kinetics dataset were comparable with the results of 2D CNNs pretrained on ImageNet, even though the results of 3D CNNs trained on the UCF101 and HMDB51 datasets were inferior to the 2D CNNs results. In still another study, Carreira et al. proposed inception [22] based 3D CNNs, which they referred to as I3D, and achieved state-of-the-art performance [2]. More recently, some works introduced ResNet architectures into 3D CNNs [9, 24], though they examined only relatively shallow ones.


\noindent
\textbf{Video Datasets:}  

\textbf{$-$ The current benchmarks are rather limited in at least one of these aspects: number of categories, samples per category, tem- poral length of each sample, diversity of video capturing conditions or environments, and the diversity of category taxonomy. We briefly review some of the most influential action datasets available.}

The HMDB-51 [17] and UCF-101 [21] datasets are currently the most successful in the field of action recognition. These datasets gained significant popularity in the early years of the field, and are still used as popular benchmarks. However, a recent consensus has emerged that indicates that they are simply not large enough for training deep CNNs from scratch [16].

A couple of years after the aforementioned datasets were introduced, larger video datasets were produced. These include ActivityNet [5], which contains 849 hours of video, including 28,000 action instances. ActivityNet also provides some additional tasks, such as untrimmed classification and detection, but the number of action instances is still on the order of tens of thousands. This year (2017), in an effort to create a successful pre-trained model, Kay et al. released the Kinetics dataset [16]. The Kinetics dataset includes more than 300,000 trimmed videos covering 400 categories. In order to determine whether it can train deeper 3D CNNs, we performed a number of experiments using these recent datasets, as well as the UCF-101 and HMDB-51 datasets.

The MPII Human Pose Dataset [2] focuses on human pose estimation, and was recently applied to action recog- nition [29]. It provides short clips (41 frames or longer) that depict human actions. Unfortunately, the distribution of video samples per category is non-uniform and biased towards some action categories.

Other huge datasets such as Sports-1M [15] and YouTube-8M [1] have been proposed. Although these databases are larger than Kinetics, their annotations are slightly noisy and only video-level labels have been as- signed. (In other words, they include frames that do not relate to target actions.) Such noise and the presence of unrelated frames have the potential to prevent these models from providing good training. In addition, with file sizes in excess of 10 TB, their scales are simply too large to allow them to be utilized easily. Because of these issues, we will refrain from discussing these datasets in this study.

large-scale video datasets: Datasets such as Sports1M [18], Kinetics [19] and AVA [27]
Crowdsourced datasets such as Charades [31] and Something-Something [9],
While KTH [29], HMDB51 [22] and UCF101 [34] have played a fundamental role in the past by inspiring the design of effective hand- engineered features for action recognition [23, 40]

Currently, the largest video dataset available is the Sports-1M dataset [16], with about 500 sports-related cat- egories, annotated by an automatic tagging algorithm. De- spite its sheer size, this dataset is structured using a some- what limited activity taxonomy, as it only focuses on sports actions. Furthermore, the automatic collection process in- troduces an undisclosed amount of label noise.

Also related to our work are the efforts to construct large- scale benchmarks for object recognition in static images. Image benchmarks such as ImageNet have spawned significant advances for com- puter vision algorithms in the related tasks. An example is the Large Scale Visual Recognition Challenge (ILSVRC), we wanna do the same at video level.

ActivityNet attempts to fill the gap in the following as- pects: a large-scale dataset that covers activities that are most relevant to how humans spend their time in.... diversity of activity taxonomy and number of classes;

\textbf{$-$ The work of [49] concatenates deep features, learned independently for the different tasks (scenes, object actions), in order to investigate possible relationships between them. However, none of this
approaches employ an end-to-end trained multi-task network for jointly solving multiple spatio-temporal problems simultaneously.  Very recently, [49] proposed a multi-task and multi-label video dataset aiming to the recognition of different visual concepts (scenes, objects, actions) which are different from our investigated tasks.}

\textbf{$-$ As mentioned before, there are lots of publicly available datasets which mostly focus on action recognition. The first ones, such as, KTH [], HMDB51 [], and UCF101 [] have inspired the design of action recognition models. To solve this issue, datasets, such as, Sports1M [], Kinetics [], and AVA [] were recently introduced. Although, such datasets have provided more training data, they are mostly focused on one task. However, HVU focuses on multi-tasks. Table \ref{table:Action_Datasets} compares video recognition datasets with HVU.}

Moreover, HVU naturally captures the long tail distribution of visual labels in the real world, whereas existing datasets are often hand designed to be well balanced. This opens the door of studying few shot learning and knowledge transfer to model the long tail [41] on a large scale video dataset.
